Learning from Failure: Training Debiased Classifier from Biased Classifier

Neural networks often learn to make predictions that overly rely on spurious correlation existing in the dataset, which causes the model to be biased. While previous work tackles this issue by using explicit labeling on the spuriously correlated attributes or presuming a particular bias type, we instead utilize a cheaper, yet generic form of human knowledge, which can be widely applicable to various types of bias. We first observe that neural networks learn to rely on the spurious correlation only when it is "easier" to learn than the desired knowledge, and such reliance is most prominent during the early phase of training. Based on the observations, we propose a failure-based debiasing scheme by training a pair of neural networks simultaneously. Our main idea is twofold; (a) we intentionally train the first network to be biased by repeatedly amplifying its "prejudice", and (b) we debias the training of the second network by focusing on samples that go against the prejudice of the biased network in (a). Extensive experiments demonstrate that our method significantly improves the training of the network against various types of biases in both synthetic and real-world datasets. Surprisingly, our framework even occasionally outperforms the debiasing methods requiring explicit supervision of the spuriously correlated attributes.

==> algorithm/pseudo.tex <==
\begin{algorithm}[t!]
\caption{Learning from Failure}
\label{alg:pseudo}
\begin{algorithmic}
\STATE $\widetilde{\mathcal{D}} \gets \mathcal{D}$
\COMMENT{\textit{Initialize dataset}}
\FOR{$i < \rm{score\_num\_iters}$}
\STATE From $\widetilde{\mathcal{D}}$, draw a mini-batch $\{(x^{(b)}, y^{(b)}): b=1,\cdots, B_{1}\}$.
\FOR{$b = 1, 2, \cdots, B_{1}$}
\STATE $\ell_{\mathtt{fail}} \gets \ell(f(x^{(b)}), y^{(b)}) - \lambda\mathcal{H}(f(x^{(b)}))$
\COMMENT{Compute loss function}
\STATE $\theta_{\mathtt{fail}} \gets \rm{Update}(\ell_\mathtt{fail}, \theta_\mathtt{fail})$ 
\COMMENT{Update network parameter}
% \STATE $\theta_\mathtt{fail} \gets \rm{Train}(\mathcal{X}, \widetilde{\mathcal{Y}}; \theta_\mathtt{fail})$
% \COMMENT{\textit{Pseudo label training}}
\STATE $y_{\mathtt{new}} \gets \argmax_{y} [f(x^{(b)})]_{y}$ 
\COMMENT{\textit{Get pseudo-label with the highest predicted probability}}
\STATE $\widetilde{\mathcal{D}} \gets \widetilde{\mathcal{D}} \setminus 
(x^{(b)}, y^{(b)}) \cup \{(x^{(b)}, y_{\mathtt{new}})\}$ 
\COMMENT{Update dataset with the new pseudo-label}
\ENDFOR
\ENDFOR
\STATE $\mathcal{E} \gets \{\ell(f_{\theta_{\mathtt{fail}}}(x), y): (x,y) \in \mathcal{D}\}$ 
\STATE $\widehat{\mathcal{D}}_{\mathtt{align}}, \widehat{\mathcal{D}}_{\mathtt{skew}} = \rm{BMM}(\mathcal{X}, \mathcal{Y}, \mathcal{E}; \theta_\mathtt{fail})$ 
\COMMENT{Seperate bias-aligned and bias-skewed samples with Beta mixture model}
\FOR{$i < \rm{main\_num\_iters}$}
\STATE From $\widehat{\mathcal{D}}_{\mathtt{align}}$, draw a mini-batch 
$\{(x^{(b)}_{\mathtt{align}}, y^{(b)}_{\mathtt{align}}): b = 1,\cdots, B_{2}\}$
\STATE From $\widehat{\mathcal{D}}_{\mathtt{skew}}$, draw a mini-batch 
$\{(x^{(b)}_{\mathtt{align}}, y^{(b)}_{\mathtt{skew}}): b = 1,\cdots, B_{2}\}$
\FOR{$b=1,2,\cdots,B_{2}$}
\STATE $\ell_{\mathtt{over}} \gets \ell(f(x_\mathtt{align}^{(b)}), y^{(b)}_\mathtt{align}) + \ell(f(x^{(b)}_\mathtt{skew}), y^{(b)}_\mathtt{skew})$
\COMMENT{Compute over-sampling loss}
\STATE $x_{\mathtt{anc}} \gets x^{(b)}_{\mathtt{skew}}$
\COMMENT{Choose the bias-skewed sample as the anchor sample}
\STATE $x_\mathtt{pos} \gets \argmax_{ x\in\widehat{\mathcal{D}}_{\mathtt{align}}\cap\{x:y=y_\mathtt{anc}\} } \|h(x) - h_\mathtt{anc}\|_2$
\COMMENT{Select positive sample for triplet loss}
\STATE $x_\mathtt{neg} \gets \argmin_{ x\in\widehat{\mathcal{D}}_{\mathtt{align}}\cap\{x:y\neq y_\mathtt{anc}\} } \|h(x) - h_\mathtt{anc}\|_2$
\COMMENT{Select negative sample for triplet loss}
\STATE $\ell_{\mathtt{tri}} \gets \max(0,  M + \lVert h_{\mathtt{anc}}- h_{\mathtt{pos}}\rVert_{2} - \lVert h_{\mathtt{anc}}- h_{\mathtt{neg}} \rVert_{2})$
\COMMENT{Compute triplet loss}
\STATE $\ell_{\mathtt{tot}} \gets \ell_{\mathtt{over}} + \gamma\ell_{\mathtt{tri}}$
\COMMENT{Compute total loss}
\STATE $\theta \gets \rm{Update}(\ell_{\mathtt{tot}}, \theta)$
\COMMENT{Update network parameter}
% \STATE Sample a mini-batch $\mathcal{B}_{\mathtt{aligned}}$ from $\widehat{\mathcal{D}}_{\mathtt{aligned}}$
% \STATE Sample a mini-batch $\mathcal{B}_{\mathtt{skewed}}$ from $\widehat{\mathcal{D}}_{\mathtt{skewed}}$
% \STATE $\mathcal{L}_{\mathtt{over}} = \mathcal{L}_{\mathtt{CE}}(\mathcal{B}_{\mathtt{aligned}}; \theta) 
% + \mathcal{L}_{\mathtt{CE}}(\mathcal{B}_{\mathtt{skewed}}; \theta)$
% \STATE $\mathcal{B}_{\mathtt{triplet}} \gets \emptyset$
% \FOR{$(x_a, y_a) \in \mathcal{B}_{\mathtt{skewed}}$}
% \STATE $x_p = \argmax_{ x\in\mathcal{B}_{\mathtt{aligned}}\cap\{x:y=y_a\} } \|h - h_a\|_2$
% \STATE $x_n = \argmin_{ x\in\mathcal{B}_{\mathtt{aligned}}\cap\{x:y\neq y_a\} } \|h - h_a\|_2$
% \STATE $\mathcal{B}_{\mathtt{triplet}} \gets \mathcal{B}_{\mathtt{triplet}}\cup\{(x_a, x_p, x_n)\}$
% \ENDFOR
% \STATE $\mathcal{L}_{\mathtt{tot}} = \mathcal{L}_{\mathtt{over}} 
% + \gamma \mathcal{L}_{\mathtt{triplet}}(\mathcal{B}_{\mathtt{triplet}}; \theta)$
% \STATE $\theta \gets \rm{Update}(\mathcal{L}_{\mathtt{tot}}; \theta)$
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> discussion.tex <==
\section{Discussions and conclusion}

There has been previous work to resolve dataset bias without explicit supervision on the bias.
\citet{geirhos2018imagenettrained} observe the presence of texture bias in the ImageNet-trained classifiers, and train shape-oriented classifier with augmented data using style transfer \citep{gatys16}.
\citet{wang2018learning} also aim to remove texture bias, using a hand-crafted module to extract bias and remove captured bias by domain adversarial loss and subspace projection.
More recently, \citet{bahng2019learning} utilize the small-capacity model to capture bias and force debiased model to learn independent feature from the biased model.
 
Such previous work mentioned above has leveraged expert knowledge, used as a substitute for explicit supervision, for a particular type of human-perceived bias. We, in a more straightforward approach, consider general properties of bias from observations on training dynamics of bias-aligned and bias-conflicting samples.
We also assume the existence of bias-conflicting samples on which the debiased model should focus, which indeed is the case in real-life application scenarios. In the end, we propose a simple yet widely applicable debiasing scheme free from the choice for form and amount of supervision on the bias. Besides, our scheme introduces only a single additional hyperparameter ($q$ in GCE), where one can enjoy simplicity in use. We expect our achievements may shed light on the nature of debiasing neural networks with minimal human supervision.

% Such previous work mentioned above has leveraged expert knowledge, used as a substitute for explicit supervision, for a particular type of human-perceived bias. We, in a more straightforward approach, consider general properties of bias from observations on training dynamics of bias-aligned and bias-conflicting samples.
% We also assume the existence of bias-conflicting samples on which the debiased model should focus, which indeed is the case in real-life application scenarios. In the end, we propose a simple yet widely applicable debiasing scheme free from the choice for form and amount of supervision on the bias. Besides, our scheme introduces only a single additional hyperparameter ($q$ in GCE), where one can enjoy simplicity in use. We expect our achievements may shed light on the nature of debiasing neural networks with minimal human supervision.


% In the end, our scheme is not only free from explicit supervision on bias but also introduces only one additional hyperparameter ($q$ in GCE, which is the same for all the experiments throughout the paper), where one can enjoy excellence in simplicity in use. We expect our achievements may shed light on the nature of debiasing neural networks with minimal human supervision.
 
%  Our proposed debiasing scheme is based on the above observations and existence of bias-conflicting samples that our debiased model should focus. From this novel yet straightforward approach, our scheme is not only free from explicit bias supervision but also introduces only one additional hyperparameter ($q$ in GCE, which is the same for all the experiments throughout the paper), where one can enjoy excellence in simplicity in use.


% While previous works rely on expert knowledge for a certain type of human-perceived bias to be free from explicit supervision, we rather utilize more general property of bias based on observations: the bias attribute that induces unintended decision rule is learned first, and samples associated with such bias have different training dynamics compared to the other samples. Our proposed debiasing scheme is based on the above observations and existence of bias-conflicting samples that our debiased model should focus on. In addition, our debiasing scheme introduces only one additional hyperparameter ($q$ in GCE, which is the same for all the experiments throughout the paper), while other methods are built on a carefully chosen set of hyperparameters (or design choices).

% \textbf{Conclusion.} In this paper, we propose a debiasing scheme, coined Learning from Failure (LfF), for training neural networks on the biased dataset without explicit supervision on the bias. Our method is based on two empirical observations on the training procedure with biased datasets. Through extensive experiments, LfF shows highly successful results on the debiased training of neural networks. 
% From these observations and method we proposed, we expect our method may shed light on the debiasing neural networks with minimal human supervision.

% \tak{
% There have been several works that attempt to resolve dataset bias problems without explicit supervision on the bias \citep{geirhos2018imagenettrained, wang2018learning, bahng2019learning}. They have leveraged expert knowledge, which can be a substitute for explicit supervision, for a particular type of human-perceived bias. We, in a more straightforward approach, design a novel debiasing scheme by utilizing general properties of bias from our novel observations: the bias attribute that induces unintended decision rule is learned first, and samples aligned with such bias have different training dynamics compared to the other samples. In the end, our scheme succeeds in training a debiased classifier in both controlled and realistic settings without explicit supervision on the bias. Additionally, our scheme introduces only one extra hyperparameter ($q$ in GCE, which is the same for all the experiments throughout the paper), where one can enjoy excellence in simplicity in use. From this novel yet straightforward observations and method we proposed, we expect our achievements may shed light on the nature of debiasing neural networks with minimal human supervision.
% }


% In this paper, we propose a debiasing scheme, coined Learning from Failure (LfF), for training neural networks on the biased dataset without explicit supervision on the bias. There have been several works that attempt to resolve dataset bias problems without explicit supervision on the bias.
% \citet{geirhos2018imagenettrained} observe the presence of texture bias in the ImageNet-trained classifiers, and train shape-oriented classifier with augmented data using style transfer.
% \citet{wang2018learning} also aim to remove texture bias, using a hand-crafted module to extract bias and remove captured bias by domain adversarial loss and subspace projection.
% More recently, \citet{bahng2019learning} utilize the small-capacity model to capture bias and force debiased model to learn independent feature from the biased model.

% While previous works rely on expert knowledge for a certain type of human-perceived bias to be free from explicit supervision, we rather focus on more general property of bias based on observations: the bias attribute that induces unintended decision rule is learned first, and samples contaminated by such bias have different training dynamics compared to the other samples.
% %Previous works attempt to be free from explicit supervision by relying on expert knowledge for a specific type of human-perceived bias. We instead focus on more general properties of bias based on observations: models learn the bias attribute first when it induces unintended decision rule, and the training dynamics depend on whether such bias resides in the samples or not.

% Our proposed debiasing scheme is solely based on the above observations and requires only one additional hyperparameter ($q$ in GCE), which is the same for all the experiments throughout the paper. Since other methods require a carefully chosen set of hyperparameters (or design choices), we expect our method may shed light on the debiasing neural networks with minimal human supervision.




==> table/action_with_groupDRO.tex <==
\begin{table}[h!]
\centering
\caption{
Class-wise action recognition accuracy on BAR evaluation set. Best performing results are marked in bold.
}
\label{tab:action}
\scalebox{0.88}{
\begin{tabular}{lccccccccc}
\toprule
\texttt{Action} & & \texttt{Climbing} & \texttt{Diving} & \texttt{Fishing} & \texttt{Racing} & \texttt{Throwing} & \texttt{Vaulting} & & {Average} 
\\
% Bias attribute & & \texttt{RockWall} & \texttt{Underwater} & \texttt{WaterSurface} & \texttt{APavedTrack} & \texttt{PlayingField} & \texttt{Sky} & &  \\
\cmidrule{1-8} \cmidrule{10-10}
Vanilla
& 
& 59.05\stdv{17.48}
& 16.56\stdv{1.58} 
& 62.69\stdv{3.64} 
& 77.27\stdv{2.62} 
& 28.62\stdv{2.95} 
& 66.92\stdv{7.25} 
& & 51.85\stdv{5.92}
% & & 50.25\stdv{1.15}

% seed 1,2,3,4
% & 57.86\stdv{14.47}
% & 16.66\stdv{1.31} 
% & 66.66\stdv{8.47} 
% & 76.51\stdv{2.62} 
% & 30.29\stdv{4.11} 
% & 69.08\stdv{7.33} 
% & & 50.84\stdv{1.50}
% \\
% Group DRO
% &
% & 80.38\stdv{2.61}
% & 51.54\stdv{8.31}
% & 81.07\stdv{6.25}
% & 78.64\stdv{2.39}
% & 21.24\stdv{2.89}
% & 77.40\stdv{3.79}
% & & 65.04\stdv{1.17}

\\

Ours
&
& \textbf{79.36}\stdv{4.79} 
& \textbf{34.59}\stdv{2.26} 
& \textbf{75.39}\stdv{3.63} 
& \textbf{83.08}\stdv{1.90} 
& \textbf{33.72}\stdv{0.68} 
& \textbf{71.75}\stdv{3.32} 
& & \textbf{62.98}\stdv{2.76}

% \cmidrule{1-8} \cmidrule{10-10}
% Ours
% &
% & 79.36\stdv{4.79} 
% & 34.59\stdv{2.26} 
% & 75.39\stdv{3.63} 
% & 83.08\stdv{1.90} 
% & 33.72\stdv{0.68} 
% & 71.75\stdv{3.32} 
% & & 62.98\stdv{2.76}

\\
\bottomrule
\end{tabular}
}
\vspace{-.1in}
\end{table}

==> table/comparison.tex <==
\begin{table}[ht!]

\centering
\caption{
Validation accuracy evaluated on the unbiased samples for the Colored-MNIST dataset with other de-biasing method of various type of supervision for bias.
}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc} 
\toprule
\multirow{2}{*}{Methods} 
& \multirow{2}{*}{Bias supervision} 
& \multicolumn{6}{c}{Bias-aligned sample ratio (\%)} 
\\
\cmidrule{3-8}
& 
& 95.0 
& 98.0 
& 99.0 
& 99.5 
& 99.7 
& 99.9 
\\
\midrule
Vanilla 
& 
& 96.91 
& 93.35 
& 87.11 
& 77.07 
& 64.14 
& 30.36 
\\
\midrule
HEX (Wang et al., 2019) 
& Type of bias 
& 85.04 & 67.04 & 52.00 & 32.69 & 21.98 & 12.65 \\
ReBias (Bahng et al., 2020) 
& Type of bias 
& 96.78 & 93.28 & 85.81 & 75.46 & 59.12 & 27.01 \\
Group DRO (Sagawa et al., 2020) 
& Label of bias 
& \textbf{97.83} & \textbf{96.21} & \textbf{93.49} & \textbf{87.27} & 80.07 & 52.14 \\
\midrule
Ours 
& 
& 96.94 & 94.10 & 93.39 & 85.54 & \textbf{82.00} & \textbf{66.70} \\
\bottomrule
\end{tabular}
}
\end{table}

==> table/method_severity_ratio_template.tex <==
\begin{table}[ht!]
\centering
\caption{
Validation accuracy evaluated on the unbiased samples and bias-skewed samples for the Colored-MNIST and Corrupted-CIFAR-10$^{1,2}$ datasets with varying difficulty of the bias attributes. Best performing results are marked in bold. 
}
\begin{tabular}{lccccccccccc}
\toprule
\multirow{2}{*}{ Method } & & \multirow{2}{*}{ Supervision  type } & & \multirow{2}{*}{ Difficulty } & & \multicolumn{6}{c}{ Skew Ratio } \\
\cmidrule{7-12}
& & & & & & 95.0 & 98.0 & 99.0 & 99.5 & 99.7 & 99.9 \\
\midrule
\multirow{4}{*}{ HEX \citep{wang2018learning} } & & \multirow{4}{*}{ \triangle } & & 1 & & - & - & - & - & - & - \\
& & & & 2 & & - & - & - & - & - & - \\
& & & & 3 & & - & - & - & - & - & - \\
& & & & 4 & & - & - & - & - & - & - \\
\hline
\multirow{4}{*}{ REPAIR } & & \multirow{4}{*}{ \triangle } & & 1 & & - & - & - & - & - & - \\
& & & & 2 & & - & - & - & - & - & - \\
& & & & 3 & & - & - & - & - & - & - \\
& & & & 4 & & - & - & - & - & - & - \\
\hline
\multirow{4}{*}{ Group DRO \citep{sagawa2019distributionally} } & & \multirow{4}{*}{ \circ } & & 1 & & - & - & - & - & - & - \\
& & & & 2 & & - & - & - & - & - & - \\
& & & & 3 & & - & - & - & - & - & - \\
& & & & 4 & & - & - & - & - & - & - \\
\hline
\multirow{4}{*}{ Vanilla } & & \multirow{4}{*}{  } & & 1 & & - & - & - & - & - & - \\
& & & & 2 & & - & - & - & - & - & - \\
& & & & 3 & & - & - & - & - & - & - \\
& & & & 4 & & - & - & - & - & - & - \\
\hline
\multirow{4}{*}{ Ours } & & \multirow{4}{*}{  } & & 1 & & - & - & - & - & - & - \\
& & & & 2 & & - & - & - & - & - & - \\
& & & & 3 & & - & - & - & - & - & - \\
& & & & 4 & & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\end{table}

==> table/ratio.tex <==
\begin{table}[t!]
\centering
\caption{
Accuracy evaluated on the unbiased samples for the Colored-MNIST and Corrupted-CIFAR-10$^{1,2}$ datasets with varying ratio of bias-aligned samples. 
}
\label{tab:ratio}
\scalebox{0.88}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{Dataset} 
& \multirow{2}{*}{Ratio (\%)} 
& \multicolumn{2}{c}{No Supervision} 
&
& \multicolumn{3}{c}{Bias Supervision} 
\\
\cmidrule{3-4}
\cmidrule{6-8}
&
& Vanilla 
& Ours 
% &  
% & Vanilla 
% & Ours 
&  
% & Vanilla 
% & Ours 
& HEX 
& REPAIR
& Group DRO
\\
\midrule
\multirow{4}{*}{\makecell{Colored\\MNIST}} 
& 95.0 
& 77.63\stdv{0.44}
& \textbf{85.39}\stdv{0.94}
% &  
% & 100.0\stdv{0.xx}
% & 80.04\stdv{0.xx}
&  
& 70.44\stdv{1.41}
& 82.51\stdv{0.59}
& 84.50\stdv{0.46}
\\
& 98.0 
& 62.29\stdv{1.47}
& \textbf{80.48}\stdv{0.45}
% &  
% & 99.90\stdv{0.xx}
% & 79.73\stdv{0.xx}
&  
& 62.03\stdv{0.24}
& 72.86\stdv{1.47}
& 76.30\stdv{1.53}
\\
& 99.0 
& 50.34\stdv{0.16}
& \textbf{74.01}\stdv{2.21}
% &  
% & 99.71\stdv{0.xx}
% & 65.04\stdv{0.xx}
&  
& 51.99\stdv{1.09}
& 67.28\stdv{1.69}
& 71.33\stdv{1.76}
\\
& 99.5 
& 35.34\stdv{0.13}
& \textbf{63.39}\stdv{1.97}
% &  
% & 99.49\stdv{0.xx}
% & 73.75\stdv{0.xx}
&  
& 41.38\stdv{1.31}
& 56.40\stdv{3.74}
& 59.67\stdv{2.73}
\\
\midrule
\multirow{4}{*}{\makecell{Corrupted\\CIFAR-10$^1$}} 
& 95.0 
& 45.24\stdv{0.22}
& \textbf{59.95}\stdv{0.16}
% &  
% & 99.00\stdv{0.xx}
% & 65.80\stdv{0.xx}
&  
& 21.74\stdv{0.27}
& 48.74\stdv{0.71}
& 53.15\stdv{0.53}
\\
& 98.0 
& 30.21\stdv{0.82}
& \textbf{49.43}\stdv{0.78}
% &  
% & 99.10\stdv{0.xx}
% & 63.40\stdv{0.xx}
&  
& 17.81\stdv{0.29}
& 37.89\stdv{0.22}
& 40.19\stdv{0.23}
\\
& 99.0 
& 22.72\stdv{0.87}
& \textbf{41.37}\stdv{2.34}
% &  
% & 98.80\stdv{0.xx}
% & 58.20\stdv{0.xx}
&  
& 16.62\stdv{0.80}
& 32.42\stdv{0.35}
& 32.11\stdv{0.83}
\\
& 99.5 
& 17.93\stdv{0.66}
& \textbf{31.66}\stdv{1.18}
% &  
% & 99.20\stdv{0.xx}
% & 59.30\stdv{0.xx}
&  
& 15.39\stdv{0.13}
& 26.26\stdv{1.06}
& 29.26\stdv{0.11}
\\
\midrule
\multirow{4}{*}{\makecell{Corrupted\\CIFAR-10$^2$}} 
& 95.0 
& 41.27\stdv{0.98}
& \textbf{58.57}\stdv{1.18}
% &  
% & 98.10\stdv{0.xx}
% & 61.00\stdv{0.xx}
&  
& 19.25\stdv{0.81}
& 54.05\stdv{1.01}
& 57.92\stdv{0.31}
\\
& 98.0 
& 28.29\stdv{0.62}
& \textbf{48.75}\stdv{1.68}
% &  
% & 98.90\stdv{0.xx}
% & 55.80\stdv{0.xx}
&  
& 15.55\stdv{0.84}
& 44.22\stdv{0.84}
& 46.12\stdv{1.11}
\\
& 99.0 
& 20.71\stdv{0.29}
& \textbf{41.29}\stdv{2.08}
% &  
% & 98.40\stdv{0.xx}
% & 47.90\stdv{0.xx}
&  
& 14.42\stdv{0.51}
& 38.40\stdv{0.26}
& 39.57\stdv{1.04}
\\
& 99.5 
& 17.37\stdv{0.31}
& \textbf{34.11}\stdv{2.39}
% &  
% & 99.60\stdv{0.xx}
% & 46.20\stdv{0.xx}
&  
& 13.63\stdv{0.42}
& 31.03\stdv{0.42}
& 34.25\stdv{0.74}
\\
\bottomrule
\end{tabular}
}
\end{table}

==> table/real.tex <==
\begin{table}[ht!]
% \begin{tabular}{ccccccccccc}
\centering
\caption{
Validation accuracy evaluated on the unbiased and bias-skewed samples for the CelebA and Biased Action dataset.
}
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Dataset} 
& \multicolumn{2}{c}{Unbiased} 
% &
% & \multicolumn{2}{c}{Aligned} 
&
& \multicolumn{2}{c}{Skewed} 
\\
\cmidrule{2-3}
\cmidrule{5-6}
% \cmidrule{9-10}
& Vanilla 
& Ours 
% &  
% & Vanilla 
% & Ours 
&  
& Vanilla 
& Ours 
\\
\midrule
CelebA
& 71.10\stdv{0.xx}
& \textbf{76.34}\stdv{0.xx}
&  
& 46.91\stdv{0.xx}
& \textbf{66.66}\stdv{0.xx}
\\
Biased Action
& -
& -
&  
& 47.88\stdv{0.xx}
& \textbf{54.06}\stdv{0.xx}
\\
\bottomrule
\end{tabular}
\end{table}
